CaT-GNN: Enhancing Credit Card Fraud Detection via Causal Temporal Graph Neural Networks

Credit card fraud poses a significant threat to the economy. While Graph Neural Network (GNN)-based fraud detection methods perform well, they often overlook the causal effect of a node's local structure on predictions. This paper introduces a novel method for credit card fraud detection, the \textbf{\underline{Ca}}usal \textbf{\underline{T}}emporal \textbf{\underline{G}}raph \textbf{\underline{N}}eural \textbf{N}etwork (CaT-GNN), which leverages causal invariant learning to reveal inherent correlations within transaction data. By decomposing the problem into discovery and intervention phases, CaT-GNN identifies causal nodes within the transaction graph and applies a causal mixup strategy to enhance the model's robustness and interpretability. CaT-GNN consists of two key components: Causal-Inspector and Causal-Intervener. The Causal-Inspector utilizes attention weights in the temporal attention mechanism to identify causal and environment nodes without introducing additional parameters. Subsequently, the Causal-Intervener performs a causal mixup enhancement on environment nodes based on the set of nodes. Evaluated on three datasets, including a private financial dataset and two public datasets, CaT-GNN demonstrates superior performance over existing state-of-the-art methods. Our findings highlight the potential of integrating causal reasoning with graph neural networks to improve fraud detection capabilities in financial transactions.

==> checklist.tex <==
\section*{AAAI Reproducibility Checklist}

This paper:
\begin{itemize}
    \item Includes a conceptual outline and/or pseudocode description of AI methods introduced(\answerYes{})
    \item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results (\answerYes{})
    \item Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper (\answerYes{})
\end{itemize}

Does this paper make theoretical contributions? (\answerYes{})

If yes, please complete the list below.
\begin{itemize}
    \item All assumptions and restrictions are stated clearly and formally. (\answerYes{})
    \item All novel claims are stated formally (e.g., in theorem statements). (\answerYes{})
    \item Proofs of all novel claims are included. (\answerYes{})
    \item Proof sketches or intuitions are given for complex and/or novel results. (\answerYes{})
    \item Appropriate citations to theoretical tools used are given. (\answerYes{})
    \item All theoretical claims are demonstrated empirically to hold. (\answerYes{})
    \item All experimental code used to eliminate or disprove claims is included. (\answerYes{})
\end{itemize}

Does this paper rely on one or more datasets? (\answerYes{})

If yes, please complete the list below.
\begin{itemize}
    \item A motivation is given for why the experiments are conducted on the selected datasets (\answerYes{})
    \item All novel datasets introduced in this paper are included in a data appendix. (\answerNA)
    \item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (\answerNA)
    \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. (\answerYes{})
    \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. (\answerYes{})
    \item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. (\answerNA)
\end{itemize}
Does this paper include computational experiments? (\answerYes{})

If yes, please complete the list below.
\begin{itemize}
    \item Any code required for pre-processing data is included in the appendix.(\answerYes{}).
    \item All source code required for conducting and analyzing the experiments is included in a code appendix. (\answerYes{})
    \item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (\answerYes{})
    \item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from (\answerYes{})
    \item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. (\answerYes{})
    \item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. (\answerYes{})
    \item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. (\answerYes{})
    \item This paper states the number of algorithm runs used to compute each reported result. (\answerYes{})
    \item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. (\answerYes{})
    \item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). (\answerYes{})
    \item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. (\answerYes{})
    \item This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. (\answerYes{})
\end{itemize}
